Measured-state conditioned recursive feasibility for stochastic model predictive control

In this paper, we address the problem of designing stochastic model predictive control (MPC) schemes for linear systems affected by unbounded disturbances. The contribution of the paper is twofold. First, motivated by the difficulty of guaranteeing recursive feasibility in this framework, due to the nonzero probability of violating chance-constraints in the case of unbounded noise, we introduce the novel definition of measured-state conditioned recursive feasibility in expectation. Second, we construct a stochastic MPC scheme, based on the introduction of ellipsoidal probabilistic reachable sets, which implements a closed-loop initialization strategy, i.e., the current measured-state is employed for initializing the optimization problem. This new scheme is proven to satisfy the novel definition of recursive feasibility, and its superiority with respect to open-loop initialization schemes, arising from the fact that one never neglects the information brought by the current measurement, is shown through numerical examples.

==> Figures/4Allbounds/0newMPC.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=7.5cm,
height=6cm,
at={(0.0in,0.0in)},
scale only axis,
xmin=-44,
xmax=44,
ymin=-44,
ymax=44,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left
]

\addplot[area legend, line width=1.0pt, draw=black, fill=blue, fill opacity=0.2, forget plot]
table[row sep=crcr] {%
x	y\\
40	-40\\
40	40\\
-40	40\\
-40	-40\\
}--cycle;

\addplot[area legend, line width=1.0pt, draw=black, fill=blue, fill opacity=0.2, forget plot]
table[row sep=crcr] {%
x	y\\
40	-27.0472086816613\\
40	2.55562386357079\\
-40	27.0472086816614\\
-40	-2.55562386357076\\
}--cycle;
\addplot [color=black, solid, line width=1pt, mark=o, mark options={solid, black}, forget plot]
  table[row sep=crcr]{%
-40	40\\
-9.3585028142666	20.7203354740707\\
5.51767264717709	8.19372389284068\\
10.5629937718162	2.25637729003613\\
10.9719102963344	-1.24026929274027\\
9.25892363096628	-3.12942432278591\\
5.99418388727221	-3.07245023961244\\
3.30928824847435	-2.00934174388728\\
1.32177595088701	-1.68212278471176\\
-0.31813900936373	-0.795751328609192\\
-1.39327410751767	-0.767041628031613\\
};
\addplot [color=black, dotted, line width=1pt, mark=o, mark options={solid, black}, forget plot]
  table[row sep=crcr]{%
-40	40\\
-4.96894666634425	30.0426357376669\\
20.5555337445424	19.8832463980677\\
35.5571229497868	10.3879896106416\\
41.3369210346659	0.764762161600457\\
37.3450705373759	-8.39145679214616\\
27.7108800449181	-10.6235760097651\\
17.9726491391822	-8.97313357609425\\
10.1890582850044	-6.26312204617795\\
5.66159763132641	-3.88253076117011\\
2.24596701224095	-2.4040733744948\\
};
\addplot [color=black, dashed, line width=1pt, mark=o, mark options={solid, black}, forget plot]
  table[row sep=crcr]{%
-40	40\\
-6.55111211004422	27.6363812407324\\
15.3349048804532	16.3144135829931\\
26.423701740268	6.24784837752746\\
27.6064577784954	-3.2970349043112\\
22.069307460015	-7.24388654598225\\
15.0810012586531	-7.36621576295183\\
8.71953394363248	-5.69299053890974\\
4.24482587905148	-3.28084749903115\\
1.93960093074201	-1.79103315183045\\
0.276478708164053	-1.17617601786355\\
};
\end{axis}
\end{tikzpicture}%
